Population synthesis of accreting white dwarfs: Rates and evolutionary pathways of H and He novae

Novae are some of the most commonly detected optical transients and have the potential to provide valuable information about binary evolution. Binary population synthesis codes have emerged as the most effective tool for modelling populations of binary systems, but such codes have traditionally employed greatly simplified nova physics, precluding detailed study. In this work, we implement a model treating H and He novae as individual events into the binary population synthesis code \binaryc. This treatment of novae represents a significant improvement on the `averaging' treatment currently employed in modern population synthesis codes. We discuss the evolutionary pathways leading to these phenomena and present nova event rates and distributions of several important physical parameters. Most novae are produced on massive white dwarfs, with approximately 70 and 55 per cent of nova events occurring on O/Ne white dwarfs for H and He novae respectively. Only 15 per cent of H-nova systems undergo a common-envelope phase, but these systems are responsible for the majority of H nova events. All He-accreting He-nova systems are considered post-common-envelope systems, and almost all will merge with their donor star in a gravitational-wave driven inspiral. We estimate the current annual rate of novae in M31 (Andromeda) to be approximately $41 \pm 4$ for H novae, underpredicting the current observational estimate of $65^{+15}_{-16}$, and $0.14\pm0.015$ for He novae. When varying common-envelope parameters, the H nova rate varies between 20 and 80 events per year.

==> individual_novae paper/README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
